AdaptiveNet: Post-deployment Neural Architecture Adaptation for Diverse Edge Environments

Deep learning models are increasingly deployed to edge devices for real-time applications. To ensure stable service quality across diverse edge environments, it is highly desirable to generate tailored model architectures for different conditions. However, conventional pre-deployment model generation approaches are not satisfactory due to the difficulty of handling the diversity of edge environments and the demand for edge information. In this paper, we propose to adapt the model architecture after deployment in the target environment, where the model quality can be precisely measured and private edge data can be retained. To achieve efficient and effective edge model generation, we introduce a pretraining-assisted on-cloud model elastification method and an edge-friendly on-device architecture search method. Model elastification generates a high-quality search space of model architectures with the guidance of a developer-specified oracle model. Each subnet in the space is a valid model with different environment affinity, and each device efficiently finds and maintains the most suitable subnet based on a series of edge-tailored optimizations. Extensive experiments on various edge devices demonstrate that our approach is able to achieve significantly better accuracy-latency tradeoffs (e.g. 46.74\% higher on average accuracy with a 60\% latency budget) than strong baselines with minimal overhead (13 GPU hours in the cloud and 2 minutes on the edge server).

==> tex/discussion.tex <==
\section{Discussions}



==> tex/measurements.tex <==
\section{Motivational Study}
\label{section:measurements}

\subsection{The Elasticity of Transformer}

\yuanchun{Show the effect of randomly dropping tokens at different layers in Transformer}


\subsection{The Influence of Execution Environment}

\yuanchun{Show the latency of the same model under different edge devices with different background services}


\subsection{The Limitation of Compression Solutions}

\yuanchun{Show why using model compression is not good enough.}

\textbf{Dynamic environment.} Models generated with compression techniques are still static, thus cannot achieve stable performance if the execution environment is dynamic (\eg multi-tenant systems like Android, Web Browser, etc.).
Dispatching model variants based on device models may ignore the variety of user-specific characteristics, \eg number of background services, device conditions, etc.

\textbf{Coarse granularity.} Many developers can only afford to generate a limited number of model variants, which is too coarse-grained to handle the vast diversity of edge environments.

\textbf{Resource consumption.} Generating fine-grained model variants using these techniques is energy consuming. For example, finding best model architecture for an edge device using neural architecture search (NAS) cost \xx .





==> tex/related_work.tex <==
\section{Discussion}\label{sec:discussion}

% Besides the relevant work in Section~\ref{section:background}, here we discuss the closely-related model scaling approaches in more detail.


% \wh{Plenty of works have been done to accelerate model inference on edge devices, including Model Scaling\cite{ding2021resrep,nestdnn,slim,us_slim,legodnn,anywidth,l1strategy}, hardware-aware Neural Architecture Search\cite{mnasnet,single_path_one_shot,proxylessnas,ofa,foxnas} , Dynamic Neural Network\cite{skipnet,early_exit,blockdrop}, efficient DNN model designing\cite{shufflenet,mbv1,mbv2,mbv3,efficientnetv1,efficientnetv2}, and system optimization for inference\cite{mistify,accudnn,xu2018deepcache,MOSAIC,ulayer}}

% \subsection{Model Scaling}


% reduce the number of blocks to accelerate model inference.
% Compared to NAS and Dynamic Neural Networks, our method does not need to train from the scratch, and the architecture of the model can be changed according to the environment, not just to the input.

% \textbf{Edge-centric approaches.} The mobile community is increasingly interested in adjusting the model size right on the target devices. This type of work is named model scaling(MS).\cite{nestdnn, slim, us_slim, legodnn, network_slimming, filter_pruning, structured_pruning} This type of work can well handle the environment diversity and dynamic with the help of runtime scheduler. Besides, the scaling process can be finished at the edge, which does not require edge data and saves a lot of maintenance efforts. However, MS only takes pruning into consideration, which limits architecture search space, leading to sub-optimal latency-accuracy trade-offs. \yuanchun{merge with above two para}

A issue that may be concerned in on-device model generation is the need of labelled edge data, which might be difficult if the data is not auto-labelled (like in many unsupervised tasks \cite{}).
Such a dataset can be generated by querying an oracle model with unlabelled edge data \cite{}. Letting the cloud send public data to the edge is also an option, although the edge data characteristics will not by utilized in this way.

Another issue we want to discuss is the relationship between AdaptiveNet and on-device learning. When the edge datasets are not big enough, on-device finetuning may lead to overfitting. AdaptiveNet, on the other hand, need not finetune after deployment, and a small dataset can be enough for searching for the optimal subnet. Besides, we can find a better start point for finetuning under the latency budget when the edge data distribution is different from the training data.



% \subsection{Neural Architecture Search}

% \wh{Hardware-aware NAS technology can select optimal model for a specific device after sufficient training. However, traditional cloud-centric Neural Architecture methods \cite{mnasnet,proxylessnas,single_path_one_shot,ofa,fbnet} often need to collect device information to search for the optimal model on the server or to build latency predictors. Fox-NAS\cite{foxnas} introduces quantization-friendly methods, but still can not directly search for the optimal subnet on device. The main reason is the limited computation resources on edge devices. Our method can directly evaluate the performance of subnets by reducing the searching cost. As a result, our method does not need to connect device information to the server and performs better when the data distribution is different from the training data. }

% \subsection{Edge-friendly Model Inference}

% \wh{Several techniques have been proposed to improve performance of DNN models on the edge, including optimizing DNN execution on heterogeneous edge devices\cite{ulayer,deepcache,MOSAIC,asymo}, designing lightweight backbones\cite{mbv1, mbv2, mbv3, shufflenet, efficientnetv1, efficientnetv2} and quantization\cite{deep_compression, haq, lqnet,bit_goes_down, int8} . These methods can accelerate model execution by better utilizing edge resources. The proposed method directly searches the optimal model on the edge. In the searching process, our method can collect information about the acceleration techniques on the edge, which will help us evaluate the subnets precisely. Consequently, our method is compatible with these edge-friendly model inference techniques.}

% Model backbones designed for mobile/edge.

% Systems Optimization for Inference.

% Model deployment/adaptation/scheduling for edges.

